Time-Robust Control for STL Specifications

We present a robust control framework for time-critical systems in which satisfying real-time constraints robustly is of utmost importance for the safety of the system. Signal Temporal Logic (STL) provides a formal means to express a large variety of real-time constraints over signals and is suited for planning and control purposes as it allows us to reason about the time robustness of such constraints. The time robustness of STL particularly quantifies the extent to which timing uncertainties can be tolerated without violating real-time specifications. In this paper, we first pose a control problem in which we aim to find an optimal input sequence to a control system that maximizes the time robustness of an STL constraint. We then propose a Mixed Integer Linear Program (MILP) encoding and provide correctness guarantees along with a complexity analysis of the encoding. We also show in two case studies that maximizing STL time robustness allows to account for timing uncertainties of the underlying control system.

==> chapters/milp.tex <==
\section{MILP ENCODING OF TIME ROBUSTNESS}

In this section we consider the right time robustness but the left time robustness is encoded analogously. 
\footnote{\color{red} @AR: Add text about Morari min time controller MILP solution and how it fails here. Add text why the formulation below is not straight-forward.}

\subsection{MILP Encoding of STL Operators}
Following Def.~\ref{def:time_rob_rec}, given the STL formula $\varphi$, the time robustness can be computed recursively on the structure of $\varphi$. 
The overall encoding of $\thetap_\varphi(\sstraj,t)$ builds on the encoding of predicates, i.e. $\thetap_{p}(\sstraj,t)$.
Note that definitions of all STL operators ($\neg$, $\wedge$, $\until_I$), except the definition of the predicates, for time robustness are the same as for the characteristic function $\chi$, see Def.~\ref{def:char_func} and the space robustness, see \cite{FainekosP09tcs,Donze10STLRob}. Thus, for these Boolean and temporal operators we can use the same MILP encoding as in \cite{raman2014model}. Briefly, since these operators are the functions of negation, $\min$ and $\max$ that can be expressed as MILP constrains, the overall encoding is straightforward. For instance, let $\varphi = \wedge_{i=1}^n \varphi_i$ and $\forall i,\ \thetap_{\varphi_i}(\sstraj,t) = r_i$. Then $\thetap_{\formula}(\sstraj,t) = r$ if and only if:
\begin{equation}
	\label{eq:conj}
	\begin{aligned}
		&r_i - M(1-b_i) \leq r \leq r_i, \ \forall i\in\{1,\ldots n\}\\
		& \sum_{i=1}^{n} b_i = 1
	\end{aligned}
\end{equation}
 where $b_i=\{0,1\}$, $i=\{1,\ldots,n\}$ are introduced binary variables and $M$ is a big-$M$ parameter\footnote{$M$ is a large positive constant, 	
 	should be at least an upper bound on all pair-wise combinations of $r_i$, $M\geq |r_i-r_j|$. For more, see the \textit{Big M method}.} 
%Constraints \eqref{eq:conj} enforce $r=\min r_i$.

Next we solve the main milestone of the overall time robustness MILP encoding, that is encoding of the predicates, i.e. $\thetap_{p}(\sstraj,t)$. 

\subsection{MILP Encoding of the Predicates} 
\label{sec:milp_pred}

Let $p\in AP$ be the predicate of interest.

\begin{enumerate}
	\item First, we construct a Boolean variable $z_t=\{0,1\}$ that corresponds to the satisfaction of the predicate $p$ at time point $t$ by trajectory $\sstraj$, i.e. $z_t=1$ if and only if $\mu(x_t)\geq 0$. Variable $z_t$ can be defined as a set of MILP constraints as follows:
	\begin{equation}
		-M(1-z_t)+\epsilon \leq \mu(x_t) \leq M z_t - \epsilon
	\end{equation}

	Note that by Def.~\ref{def:char_func}$, \chi_p(\sstraj,t)=\sign \mu(x_t)$, therefore, it can be encoded as $\chi_{p}(\sstraj,t) = 2 z_t -1$.
	
	\item\label{it:l}  Recall that
	\begin{align*}
		\thetap_p(\sstraj,t) = \chi_p(\sstraj, t)\cdot
		\max\{\tau\geq0\ :\ &\forall t'\in[t,t+\tau],\\ &\chi_p(\sstraj,t')=\chi_p(\sstraj,t)\}. 
	\end{align*}
	Since $\chi_p(\sstraj,t) \in\{-1,+1\}$ there exist two disjoint possibilities for $\thetap_p$ which in terms of $z_t$ can be written as:
	\begin{equation*}
			\thetap_p(\sstraj,t)\! =\!\!  
			\begin{cases}
			\max\{\tau:\forall t'\in[t,t+\tau], z_{t'}=1\} ,&\text{if } z_t=1 \\
			-\max\{\tau:\forall t'\in[t,t+\tau], z_{t'}=0\},&\text{if } z_t=0 \\
			\end{cases}
	\end{equation*}
	In other words, if at time point $t$, $z_t=1$, one can count the maximum number of sequential $z_{t'}=1$ to the right to calculate $\thetap_p(\sstraj,t)$. On the other hand, if $z_t=0$, then counting 0s to the right will define the time robustness value. 
	
%	\item
%	Consider the counter $l_t$ that enumerates the number of consecutive time intervals in the future for which $\chi_p(\sstraj, t)$ keeps its value unchanged. 
%	By the definition, the right time robustness is 
%	$\thetap_p(\sstraj,t) = \chi_p(\sstraj, t) \cdot l_t $. Since $\chi\in\{-1,+1\}$ then depending on the value of $\chi_p(\sstraj, t)$, $\thetap_p(\sstraj,t) = \pm l_t$.
	
	\item\label{it:c} We construct the counter $c_t^1$ that counts the maximum number of sequential $z_{t'}=1$ to the right ($t'\geq t$). Analogously, we construct another counter $c_t^0$ that counts sequential $z_{t'}=0$. Both can be defined recursively as following:
	\begin{align}
		\label{eq:c1}
		c_t^1 &= (c_{t+1}^1+1) \cdot z_t, \qquad\qquad\ \, c^1_{H+1}=0\\
		\label{eq:c0}
		c_t^0 &= (c_{t+1}^0-1) \cdot (1-z_t),
		\qquad c^0_{H+1}=0
	\end{align} 
	Note that counters are defined backwards: from $t=H+1$ to $t=0$, so 
	while the length of trajectory $\sstraj$ is $H+1$,
	the lengths of $c_t$ sequences are $H+2$.
	
	\item Next, in order to count the number of \textit{intervals} instead of \textit{time steps}, we need to reduce the obtained counter values by 1 in magnitude:
	\begin{align*}
		l_t^1 &= c_t^1 - z_t, \qquad\quad\ \, t=1,\ldots,H\\
		l_t^0 &= c_t^0 + (1-z_t),\quad t=1,\ldots,H
	\end{align*}

	\item Finally, using the fact from step \ref{it:l}) that two possibilities of $z_t$ being 1 or 0 are disjoint, the right time robustness $\theta_p(\sstraj,t)$ is defined as:
	\begin{equation*}
		\thetap_p(\sstraj,t) = l_t^1 + l_t^0.
	\end{equation*} 
\end{enumerate}

\begin{table}[t!]
	\renewcommand{\arraystretch}{1.5}
	\setlength{\tabcolsep}{3pt}
	\centering
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
		\hline
		$t$   & 0 & 1  & 2  & 3 & 4 & 5 & 6 & 7 & 8 \\ \hline
		\hline
		$z_t$ & 1 & 1 & 0 & 1 & 1 & 1 & 0 & 0 &  \\ \hline
		$c^1_t =(c_{t+1}^1+1) \cdot z_t,\  c^1_{H+1}=0$    & 2 & 1  &  0 & 3  &  2 &  1 &  0 & 0  & 0  \\ \hline
		$c_t^0 = (c_{t+1}^0-1) \cdot (1-z_t),
		\ c^0_{H+1}=0$    &  0  &  0  & -1  & 0  & 0  & 0  & -2  &  -1 & 0  \\ \hline
		$l^1_t = c_t^1 - z_t$    &  1   & 0  & 0  & 2  & 1  & 0  & 0  & 0  &  \\ \hline
		$l^0_t = c_t^0 + (1- z_t)$    &  0  &  0  & 0  & 0  & 0  & 0  & -1  & 0  &   \\ \hline \hline
		$\thetap_p(t) = l^1_t + l^0_t$ & 1   & 0  & 0  & 2  & 1  &  0 & -1  & 0 &   \\ \hline
	\end{tabular}
	\vspace{0pt}
	\caption{MILP encoding of $\thetap_p(\sstraj,t)$ from Example~\ref{ex:running}.}
	\label{tab:exmp_theta}
\end{table}

\begin{exmp}[continues=ex:running]
%	\label{exmp:theta}
Consider again the signal $\sstraj$ and predicate $p$ shown in Fig.~\ref{fig:ex1}.
In Table~\ref{tab:exmp_theta} we consider a step-by-step estimation of the right time robustness for predicate $p$ following the MILP encoding procedure described in \ref{sec:milp_pred}.
On the other hand, using Def.~\ref{def:time_rob_rec}, one can check that $\thetap_p(\sstraj) = (1, 0, 0, 2, 1, 0, -1, 0)$. MILP encoding procedure leads to the same result as estimation by the definition.
\end{exmp}


\textit{Remark.} Constraints \eqref{eq:c1}-\eqref{eq:c0} are specified using a product of the integer and boolean variables. Using Lemma~\ref{lemma:xz} below we show that such product can be expressed as MILP constraints.
\begin{lemma}[Linearization of the Boolean-Integer Product]
	\label{lemma:xz}
	Let $b$ be a Boolean variable and let $x$ be an integer variable such that lower and upper bounds are known constants, $x_l\leq x\leq x_{u}$. The expression 
	$y=b\cdot x$ can be written as a set of mixed-integer linear (MIL) constraints, i.e:
	\begin{equation}
		\label{eq:inq}
		y=x\cdot b \quad \Longleftrightarrow\quad
		\begin{aligned}
			x_lb\leq\  &y\leq x_{u} b \\
			x - x_{u}(1-b) \leq &y \leq x- x_l(1-b).
		\end{aligned}
	\end{equation}
\end{lemma}



	
We summarize the main properties of the above MILP formulation in the following proposition.
\begin{prop}
	\begin{enumerate}
		\item Problem~\ref{prob:synthesis} is equivalent to an MILP (ref \#). Therefore, it is NP-hard.
		\item MILP (ref \#) is a function of $O(H\cdot |AP|)$ binary and $O(H\cdot |\varphi|)$ continuous variables, where $H$ is the time horizon and $|\varphi|$ is the number of operators in the formula $\varphi$.  
	\end{enumerate}
\end{prop}


\begin{table*}[t!]
	\renewcommand{\arraystretch}{1.3}
	%\setlength{\tabcolsep}{1.5pt}
	\centering
	\begin{tabular}{l|c|cc|cc|c}
		\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Mission}}} &
		\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\# Constraints}}} &
		\multicolumn{2}{c|}{\textbf{\# Variables}} &
		\multicolumn{2}{c|}{\textbf{Computation time}} &
		\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Time Rob., $\thetap_{\formula}(\sstraj,0)$}}} \\
		\multicolumn{1}{c|}{} &
		\multicolumn{1}{c|}{} &
		\multicolumn{1}{c}{\textbf{Boolean}} &
		\multicolumn{1}{c|}{\textbf{Integer}} &
		\multicolumn{1}{c}{\textbf{YALMIP}} &
		\multicolumn{1}{c|}{\textbf{Solver}} &
		\multicolumn{1}{c}{} \\ \hline
		$\varphi_2$	Raman paper & 647 & 74 & 189 & 0.29 &0.16 & 26  \\
		$\varphi_3$	Raman paper & 628 & 177 & 119 & 0.31 & 0.19 & 10 \\
		\hline
		Case study 1, Eq.\eqref{eq:ex_drone} &2447  &224  &502  &0.41  & 0.34&23 \\ \hline
		Case study 2, Eq.\eqref{eq:mission2}& 8794 & 2750 & 858 & 0.82 & 49.69&14 \\
		Case study 2 with velocity constraint, Eq.\eqref{eq:vel_constr} & 9034 & 2750 & 858 & 0.88 &29.08 & 14 \\
		Case study 2 with velocity constraint on $y$, & 8914 & 2750 & 858 & 0.82 &66.19 & 14 \\
		Case study 2: Feasibility formulation, $\theta_\varphi(\sstraj,0)=5$, Fig.~\ref{fig:ex_agents(t)}(a) & 8795 & 2750 &858  & 0.81 & 2.12 & 5\\
		Case study 2: Feasibility formulation, $\theta_\varphi(\sstraj,0)=1$, Fig.~\ref{fig:ex_agents(t)}(b) & 8795 & 2750 &858  & 0.85 & 1.02 & 1
	\end{tabular}
	\caption{Results. Maybe include Computation times (mean and standard deviation).}
	\label{tab:experiments}
\end{table*}
%%%%%%%%%%%%%%%%%%%


==> chapters/theorems.tex <==
\section{PROPERTIES OF TIME ROBUSTNESS}

\begin{theorem}
	\label{thm:sat}
	For an STL formula $\varphi$, trajectory $\sstraj:\TDom \rightarrow X$ and some time $t\in\TDom$, the following results hold: 
	\begin{enumerate}
		\item\label{i1} $\theta^{\bowtie}_\varphi(\sstraj,t) > 0 \quad\, \Longrightarrow\ \chi_\varphi(\sstraj,t)= +1$
		\item\label{i2} $\theta^{\bowtie}_\varphi(\sstraj,t) < 0 \quad\, \Longrightarrow\ \chi_\varphi(\sstraj,t)= -1$
		\item\label{i3} $\chi_\varphi(\sstraj,t)= +1 \  \Longrightarrow\ 
		\theta^{\bowtie}_\varphi(\sstraj,t) \geq 0$
		\item\label{i4} $\chi_\varphi(\sstraj,t)= -1 \  \Longrightarrow\ 
		\theta^{\bowtie}_\varphi(\sstraj,t) \leq 0$ 
	\end{enumerate}
\end{theorem}
Note that equivalence $\theta^{\bowtie}_\varphi(\sstraj,t) \geq 0 \Longleftrightarrow \chi_\varphi(\sstraj,t)= +1$ does not hold\footnote{Equivalence $\theta^{\bowtie}_\varphi(\sstraj,t) \leq 0 \Longleftrightarrow \chi_\varphi(\sstraj,t)= -1$ does not hold either, same reasoning applied.} since when $\theta^{\bowtie}_\varphi(\sstraj,t) =0$ we cannot determine if the formula is satisfied or violated. 

\begin{exmp}[continues=ex:running] $\thetap_p(\sstraj,1)=\thetap_p(\sstraj,2)=0$ but $\chi_p(\sstraj,1)= +1 \not= \chi_p(\sstraj,2)= -1$.
\end{exmp}

\begin{theorem}
	\label{thm:theta_chi} 
	For an STL formula $\varphi$, discrete-time trajectory $\sstraj:\TDom \rightarrow X$ and some time $t\in\TDom$, the following result holds:
	\begin{equation}
	\theta^{\bowtie}_\varphi(\sstraj,t) = i \ \Longrightarrow\ \forall h\in[0,\,|i|\,],\ \chi_\varphi(\sstraj,t\bowtie h)=\chi_\varphi(\sstraj,t)
	\end{equation}
\end{theorem}
	 
Note that the implication other way around does not hold nor it follows that $\chi_\varphi(\sstraj,t+i+1)\not=\chi_\varphi(\sstraj,t)$.
		
\begin{exmp}[continues=ex:running]
	Take again a look at Fig.~\ref{fig:ex1}.
	Let $\varphi=p\vee q$. Then $\thetap_{\varphi}(\sstraj,0)=\max(\thetap_{p}(\sstraj,0), \thetap_{q}(\sstraj,0))= 4$, so $i=4$. It is easy to check that indeed 
	$\chi_\varphi(\sstraj,0)=\ldots=\chi_\varphi(\sstraj,4)=+1$. 
	On the other hand, $\chi_\varphi(\sstraj,5)=+1$ as well, so $\chi_\varphi(\sstraj,t+i+1)=\chi_\varphi(\sstraj,t)$.
	Also, though $\chi_\varphi(\sstraj,0)=\ldots=\chi_\varphi(\sstraj,5)$, $\thetap_{\varphi}(\sstraj,0)\not= \pm 5$.
\end{exmp}

Interpretation of Thm.~\ref{thm:theta_chi} sounds as {\color{red} (@Lars, help me here with formal definitions of \textit{individ shifts}.)}:
If $\theta_\varphi(\sstraj,t)=s$ 
		then for any signal $\sstraj'$ obtained from $\sstraj$ by shifting \textbf{any} of the sub-signals to the left by less than or equal to $s$, we have $\chi_{\varphi}(\sstraj,t)=\chi_{\varphi}(\sstraj',t)$.
		Also there exists a shifting scheme where at least one of the sub-signals is shifted by $s+1$ and other by less than or equal to $s+1$, such that the satisfaction is guaranteed to change, i.e. $\chi_{\varphi}(\sstraj,t)\not=\chi_{\varphi}(\sstraj',t)$.
		In other words, $\theta$ defines the max possible shifts to the left of individual signals $p_i$. 



\begin{theorem}
	\label{thm:theta_theta}
	For an STL formula $\varphi$, trajectory $\sstraj:\TDom \rightarrow X$ and some time $t\in\TDom$, the following results hold:
	\begin{itemize}
		\item $\theta^{\bowtie}_\varphi(\sstraj,t) = i> 0 \ \Longrightarrow\ 
		\forall h\in[0,i],\ \theta^{\bowtie}_\varphi(\sstraj,t \bowtie i) \geq i-h$.
		\item $\theta^{\bowtie}_\varphi(\sstraj,t) = i< 0 \ \Longrightarrow\ 
		\forall h\in[i,0],\ \theta^{\bowtie}_\varphi(\sstraj,t \bowtie i) \leq i+h$.
	\end{itemize}
\end{theorem}
Note only inequality is implied, equality does not hold.
%e.g.\footnote{Same applies to $i<0$: $\thetap_\varphi(\sstraj,t) = i< 0 \ \not\!\!\Longrightarrow\ 
%	\forall h\in[i,0],\ \thetap_\varphi(\sstraj,t+i) = i+h.$.}:
%\begin{equation}
%	\thetap_\varphi(\sstraj,t) = i> 0 \ \not\!\!\Longrightarrow\ 
%	\forall h\in[0,i],\ \thetap_\varphi(\sstraj,t+i) = i-h.
%\end{equation} 

\begin{exmp}[continues=ex:running]
Recall that though $\thetap_{\varphi=p\vee q}(\sstraj,0)=4$, $\thetap_{\varphi}(\sstraj,3)=2\not=1$. Therefore, $\thetap_\varphi(\sstraj,t) = i> 0 \ \not\!\!\Longrightarrow\ 
\forall h\in[0,i],\ \thetap_\varphi(\sstraj,t+i) = i-h$.
\end{exmp}



\begin{definition}
Recall that formula $\varphi$ is built upon a set of predicates $AP=\{p^{(1)},\ldots,p^{(L)}\}$. For a given predicate $p\in AP$ and a system trajectory $\sstraj = (x_0,x_{1}\ldots,x_{H})\in\SigSpace$, we call the sequence $\mathbf{p}=(p_0,\ldots,p_H)$ a \textit{predicate sub-trajectory}.
	\end{definition}

Let us assume that for the system
trajectory $\sstraj$ 
and given formula $\varphi$ with $len(\varphi)=H_\varphi \leq H$,
%\footnote{Otherwise, $\sstraj\models\varphi$ is ill defined.}, 
$\thetap_\varphi(\sstraj,0)= i$.  
We next define the set of signals $\mathbf{s}$ that can be obtained from $\sstraj$ by shifting one or several predicate sub-trajectories by at most $|i|$ to the left, i.e.:\footnote{Precisely speaking, it should be $\forall h\in[0,\ \min(|i|,\ H-H_\varphi)]$. Check this throughout the paper.}
\begin{equation}
	\label{eq:S}
	\begin{aligned}
		\mathbb{S}_{\sstraj}:=\{\mathbf{s}=(s_0,\hdots,s_{H-h})\ |
		%s_k\in X
		&\ \forall h\in[0,|i|], \ 
		\forall t\in[0,H-h], \\
		&\ \forall AP'\subseteq AP,\ \forall p\in AP',\\  
		&\ \chi_p(\mathbf{s}, t )=\chi_p(\sstraj, t+h)\}.
	\end{aligned}
\end{equation}  

%If I'm not wrong, then it shold hold that all signals $\mathbf{s}\in \mathbb{S}$ are such that $\chi_\varphi(\mathbf{s}, 0 )=\chi_\varphi(\sstraj, 0 )$. I suspect that this is what  Theorem 2 in \cite{Donze10STLRob} wants to say. I suppose we could write an inductive proof for that based on (5) and (6) and then follow the recursion in (7), (8), and (9).

\begin{theorem}
	\label{thm:ind_shift}
	Let $\varphi$ be such that $len(\varphi)\le H$ and let $\sstraj$ be such that $\thetap_\varphi(\sstraj,0)= i$. Then $\forall\mathbf{s}\in \mathbb{S}_\sstraj$, $\chi_\varphi(\mathbf{s}, 0 )=\chi_\varphi(\sstraj, 0 )$. 
\end{theorem}

\textcolor{red}{Summary of what's missing or wrong in Donze: 1) Definition has a typo, 2) No proof for theorem, 3) Theorem doesn't mention the absolute value that has to be taken to shift signal from the calculated time robustness.}


